A Comprehensive Evaluation of Large Language Models on Legal Judgment Prediction

Large language models (LLMs) have demonstrated great potential for domain-specific applications, such as the law domain. However, recent disputes over GPT-4's law evaluation raise questions concerning their performance in real-world legal tasks. To systematically investigate their competency in the law, we design practical baseline solutions based on LLMs and test on the task of legal judgment prediction. In our solutions, LLMs can work alone to answer open questions or coordinate with an information retrieval (IR) system to learn from similar cases or solve simplified multi-choice questions. We show that similar cases and multi-choice options, namely label candidates, included in prompts can help LLMs recall domain knowledge that is critical for expertise legal reasoning. We additionally present an intriguing paradox wherein an IR system surpasses the performance of LLM+IR due to limited gains acquired by weaker LLMs from powerful IR systems. In such cases, the role of LLMs becomes redundant. Our evaluation pipeline can be easily extended into other tasks to facilitate evaluations in other domains. Code is available at https://github.com/srhthu/LM-CompEval-Legal

==> emnlp2023-latex/chapters/1_intro_yx.tex <==
Large language models have achieved a great success in various Natural Language Processing (NLP) tasks~\citep{brown2020language,wei2022chain,kojima2022zero-shot-reasoner}, while there are some disputes over the potential to domain-specific applications~\citep{martinez2023re-eval}. Focusing on the law domain, the leading LLM, GPT-4, was claimed to pass the Uniform Bar Exam (UBE) with a 90th percentile score. Although inspiring, however, this result was pointed out to be over estimated. This raises an interesting question: how exactly LLMs perform in various settings of real-world legal tasks?

In this paper, we design practical baseline solutions based on LLMs and systematically investigate their law competence, to shed light on other domains as well. We attribute the main issues of previous benchmark as follows. First, UBE is too general and not subject to any legal jurisdictions~\citep{martinez2023re-eval}.
Second, in real-world applications, there are not only multi-choice but also open questions. Using multi-choice questions only may be not comprehensive enough, while open-ended answers are difficult to evaluate. Third, specifically in but not limited to common law, similar cases are always introduced as evidence to support expertise reasoning, which are typically ignored.

For the first challenge, we choose legal judgment prediction (LJP) as the example task for investigation. It is a real-world problem to determine charges committed by defendants under a juridical system. LJP is typically formulated as an classification task to predict the most possible one from a list of pre-defined charges. Note that our evaluation pipeline can be easily extended into other tasks as well. Then, for the second and third challenges, we design four settings derived from two work scenarios of LLMs. 
In the two scenarios, LLMs can either 1) \textbf{work alone}, assuming all domain knowledge is implicitly stored using parameters, or 2) \textbf{coordinate with an information retrieval (IR) system}, which is used to retrieve similar cases.
Thus, for each scenario, we testify the law competence of LLMs on LJP in both forms of multi-choice and open questions.

For benchmarking, we 
These similar cases then benefit expertise reasoning by 1) suggesting \textit{label candidates} and 2) providing \textit{similar demonstrations} \citep{liu2021good-examples} for in-context learning. 
The two usages of the IR system constitutes two dimensions of evaluation settings. The setting without label candidates is denoted as free generation (\textbf{Free}) and with label candidates as multi-choice questions (\textbf{Multi}). Similarly, adding similar demonstrations converts the setting from zero-shot (\textbf{ZS}) to few-shot (\textbf{FS}) prompting.
We evaluated five up-to-date LLMs including the powerful yet close-source GPT-3 family, ChatGPT and GPT-4, and open-source LLMs including Vicuna, ChatGLM and BLOOMZ.
We adopt a Chinese LJP dataset, namely CAIL \citep{xiao2018cail2018}, which contains 10K criminal law cases under 112 charges\footnote{After filtering rare charges}. 

In experiments, we first examines the effects of two usages of IR systems for providing domain knowledge (Section 4). 
We find that both label candidates and similar cases can activate LLM to recall acquired domain knowledge, resulting in significant improvements. In contrast, fixed cases hardly show such effects.
Then comes in-depth analysis of label candidates (Section 5) and similar cases (Section 6). 
For label candidates, we propose the metric of self consistency to indicate the confidence of LLMs into generated tokens and observe a high consistency after introducing label candidates (Section 5.1). We then inspect the influence of the failure of IR systems on suggesting the ground truth labels (Section 5.2) and ablate a setup to ask LLM's opinions about each label one by one.
For similar cases, we explore the effects of number of similar demonstrations (Section 6.1). In the ablation study (Section 6.2), we find that false case-charge combinations do not mislead LLMs, which indicates that LLMs mainly rely on previous knowledge for expertise reasoning.
Finally, we explain the paradox (Section 7) of enhancing LLM with powerful IR systems. We reveal that when the capability IR systems exceed a threshold, LLMs are no longer needed as they underperform IR systems even with their help.

We summarize the main contributions in three aspects:
\begin{itemize}
    \item We propose a new benchmark, LJP that requires expertise reasoning, to evaluate the law competence of LLMs.
    \item We propose four evaluation settings to measure the performance of LLMs that work alone and coordinate with an IR system as an extra tool.
    \item Extensive experiments of 5 LLMs on the task of legal judgment prediction facilitate the understanding of expertise reasoning and provide an empirical experience of harnessing LLMs for expertise reasoning.
\end{itemize}

==> emnlp2023-latex/chapters/2_related_work.tex <==

\subsection{Large Language Models}

Language models are pre-trained on large corpus to acquire general knowledge ranging from linguistics to world knowledge \citep{raffel2020t5} that benefits natural language processing tasks. Language models, such as BERT \citep{devlin2018bert} and its followers \citep{liu2019roberta,he2020deberta}, are usually adapted to NLP tasks by domain specific fine-tuning. Recently, scaling to 175B parameters, GPT-3 \citep{brown2020language} exhibited the ability of in-context learning by simply generating following tokens to complete NLP tasks conditioned on a few task demonstrations. This work has drawn great attention to scaling language models and the emergent abilities \citep{wei2022emergent} of LLMs. 

\textbf{Scaling} Inspired by GPT-3, more LLMs have been proposed, e.g., PaLM \citep{chowdhery2022palm}, LAMDA \citep{thoppilan2022lamda}, GPT-NEOX \citep{black2022gptneox}, Gopher \citep{rae2021gopher}, OPT \citep{zhang2022opt} and BLOOM \citep{scao2022bloom}. \citet{hoffmann2022chinchilla} trained the compute-optimal LLM, namely Chinchilla, of same computing budget as Gopher but smaller model size on more tokens. Instead adopting a causal decoder architecture like GPT-3, several LLMs also tried other architectures \citep{zhao2023llm-survey}, e.g., encoder-decoder by T5\citep{raffel2020t5} and prefix decoder by GLM \citep{du2022glm}. More recent LLMs has employed various improvements over the Transformer backbone \citep{vaswani2017attention}. For example, the open-source LLaMA \citep{touvron2023llama} used rotary positional embeddings \citep{su2021roformer} and Flash attention \citep{dao2022flashattention} for efficiency.

\textbf{Emergent ability} The exploration of the prompting paradigm has uncovered various emergent abilities of LLMs. In addition to few-shot prompting of GPT-3, \citet{wei2022chain} showed that LLMs can do mathematical reasoning prompted with chain-of-thought exemplars. \citet{kojima2022zero-shot-reasoner} further demonstrated that such reasoning pattern can also be elicited by heuristic instructions like "\textit{let's think step by step}".

\textbf{Supervised fine-tuning} LLM's ability can be further advanced by supervised fine-tuning. For example, instruction tuning \citep{wei2021finetuned}

%the capacity of LLM are boosted by scaling and supervised fine-tuning.
%Scaling: T5, GPT-3, PaLM, GPT-NeoX, Gopher, Chinchilla, Opt, BLOOM, GLM, Claude, LLaMA,
% Supervised fine-tuning: FLAN, InstructGPT, T0, Flan-T5, mT0 and Bloomz, Alpaca, Vincuna LIME


\subsection{In-context learning}
Early: classification, MetaICL, channel prompting

self consistency, CoT, least-to-most, compositions gap, zero-shot reasoner

\subsection{Legal Judgment Prediction}
dataset: cail, echr
method: topojudge, neural judge
explanability: deconfouding

